Span-Oriented Information Extraction -- A Unifying Perspective on Information Extraction

Information Extraction refers to a collection of tasks within Natural Language Processing (NLP) that identifies sub-sequences within text and their labels. These tasks have been used for many years to link extract relevant information and to link free text to structured data. However, the heterogeneity among information extraction tasks impedes progress in this area. We therefore offer a unifying perspective centered on what we define to be spans in text. We then re-orient these seemingly incongruous tasks into this unified perspective and then re-present the wide assortment of information extraction tasks as variants of the same basic Span-Oriented Information Extraction task.

==> table/token_classification/binary.tex <==
{
\begin{tabular}{@{}l ccc c ccc c ccc@{}}
\toprule
X | Stonyfield & Organic & Kids & Yogurt \\
\midrule
Entity Disambiguation (ED) & Y & Entity & Tim Cook, Texas \\

\bottomrule
\end{tabular}
}

==> table/tradeoffs.tex <==
\resizebox{\columnwidth}{!}{%
{
\begin{tabular}{@{}l ccc c ccc c ccc@{}}
\toprule
& complexity & examples & \multicolumn{3}{c}{features} & \multicolumn{2}{c}{special cases} &\\
\toprule
Transformation & \# of inst. & pos./neg. for Fig~\ref{fig:token_classification_binary} & token embed. & span embed. & span class rep. & nested & discontinuous &\\
\midrule
Sequential Labeling  & $O(1)$ & 4/5 & \checkmark & \\
Token Prototype  & $O(1)$ & 4/5 & \checkmark \\ 
Token-pair Classification & $O(1)$ & 4/77 & \checkmark & & & \checkmark & \checkmark   \\
Span Classification & $O(1)$ & 3/32 & & \checkmark & \checkmark & \checkmark \\
Span Locating & $O(K)$ & 3/0 & \checkmark &  & \checkmark & \checkmark\\
Span Generation  & $O(N)$ & 6/9 & \checkmark &  & \checkmark &  \\

\bottomrule
\end{tabular}
}
}

==> table/transformation.tex <==
%\resizebox{\columnwidth}{!}{%

